Automatic Perturbation Analysis for Scalable Certified Robustness and Beyond

Linear relaxation based perturbation analysis (LiRPA) for neural networks, which computes provable linear bounds of output neurons given a certain amount of input perturbation, has become a core component in robustness verification and certified defense. The majority of LiRPA-based methods focus on simple feed-forward networks and need particular manual derivations and implementations when extended to other architectures. In this paper, we develop an automatic framework to enable perturbation analysis on any neural network structures, by generalizing existing LiRPA algorithms such as CROWN to operate on general computational graphs. The flexibility, differentiability and ease of use of our framework allow us to obtain state-of-the-art results on LiRPA based certified defense on fairly complicated networks like DenseNet, ResNeXt and Transformer that are not supported by prior works. Our framework also enables loss fusion, a technique that significantly reduces the computational complexity of LiRPA for certified defense. For the first time, we demonstrate LiRPA based certified defense on Tiny ImageNet and Downscaled ImageNet where previous approaches cannot scale to due to the relatively large number of classes. Our work also yields an open-source library for the community to apply LiRPA to areas beyond certified defense without much LiRPA expertise, e.g., we create a neural network with a probably flat optimization landscape by applying LiRPA to network parameters. Our opensource library is available at https://github.com/KaidiXu/auto_LiRPA.

==> conclusions.tex <==
\section{Conclusions}
Linear Relaxation based Perturbation Analysis (LiRPA) was originally developed for robustness verification of neural networks to provide provable output bounds. Existing efforts on this field are largely fragmented and researchers typically need to build the bounds on their own to adapt LiRPA based techniques to a new architecture~\citep{zugner2019certifiable,ko2019popqorn,shi2020robustness}. 
Additionally, the lack of a general and easy-to-use tool and the relatively cumbersome bound derivation process prevent the application of LiRPA for general machine learning audience and the industry. Our work generalizes LiRPA based algorithms to its most general form for general computational graphs, and our framework allows automatic and differentiable bound computation which enables LiRPA as a toolbox for machine learning researchers and practitioners who are not experts on verification. 
When used for certified defense training, our framework enables the loss fusion technique which significantly reduces time complexity of existing similar approaches, and outperforms previous works on large datasets like downscaled ImageNet. 
We also demonstrate potential usage of LiRPA beyond verification and certified defense. The generality, flexibility, efficiency and ease-of-use of our proposed framework facilitate the adoption of LiRPA based provable methods for other machine learning problems beyond robustness verification.

